TWLV-I: Analysis and Insights from Holistic Evaluation on Video Foundation Models

In this work, we discuss evaluating video foundation models in a fair and robust manner. Unlike language or image foundation models, many video foundation models are evaluated with differing parameters (such as sampling rate, number of frames, pretraining steps, etc.), making fair and robust comparisons challenging. Therefore, we present a carefully designed evaluation framework for measuring two core capabilities of video comprehension: appearance and motion understanding. Our findings reveal that existing video foundation models, whether text-supervised like UMT or InternVideo2, or self-supervised like V-JEPA, exhibit limitations in at least one of these capabilities. As an alternative, we introduce TWLV-I, a new video foundation model that constructs robust visual representations for both motion- and appearance-based videos. Based on the average top-1 accuracy of linear probing on five action recognition benchmarks, pretrained only on publicly accessible datasets, our model shows a 4.6%p improvement compared to V-JEPA (ViT-L) and a 7.7%p improvement compared to UMT (ViT-L). Even when compared to much larger models, our model demonstrates a 7.2%p improvement compared to DFN (ViT-H), a 2.7%p improvement compared to V-JEPA (ViT-H) and a 2.8%p improvement compared to InternVideo2 (ViT-g). We provide embedding vectors obtained by TWLV-I from videos of several commonly used video benchmarks, along with evaluation source code that can directly utilize these embeddings. The code is available at https://github.com/twelvelabs-io/video-embeddings-evaluation-framework.

==> tables/retrieval.tex <==
% text to video search
\begingroup
\begin{table}
 \centering
  \caption{\textbf{Zero-shot text-to-video retrieval.} }
\resizebox{0.7\linewidth}{!}{
 \begin{tabular}{l|cc|cc|cc}
  \hline
  \multirow{2}{*}{Method} & \multicolumn{2}{c|}{MSR-VTT} & \multicolumn{2}{c|}{MSVD} & \multicolumn{2}{c}{Activity-Net}\\ 
               & R@1   & R@5   & R@1   & R@5   & R@1   & R@5   \\ \hline
CLIP4CLIP-B    & 32.0  & 57.0  & 38.5  & 66.9  & -     & -     \\
InternVideo-L  & 40.7  & -     & 43.4  & -     & 30.7  & - \\
UMT-L 17M      & 42.6  & 64.4  & 49.9  & 77.7  & 42.8  & 69.6  \\ 
LanguageBind-H & 44.8  & 70.0  & 53.9  & 80.4  & 41.0  & 68.4 \\
\rowcolor{tl!50} \adjustbox{valign=c}{\includegraphics[width=0.02\linewidth]{tables/logo.png}} Ours  & \textbf{49.4} & \textbf{73.5} & \textbf{61.3} & \textbf{89.2} & \textbf{55.4} & \textbf{82.6} \\ \hline
VideoCoCa-g    & 34.3  & 57.8  & -   & -     & 34.5  & 63.2  \\
VideoPrism-g   & 39.7  & 63.7  & -   & - & 52.7 & 79.4 \\ %  52.7 & 77.2
InternVideo2\textrm{-6B} & 55.9 & -    & 59.3 & - & 63.2 & - \\ \hline
 \end{tabular}
}
 \label{tab:ret_t2v}
\end{table}
\endgroup

% text to image search
\begingroup
\begin{table}
\begin{minipage}{0.5\textwidth}
\centering
 \centering
  \caption{\textbf{Zero-shot text-to-image retrieval. } }
\resizebox{\linewidth}{!}{
 \begin{tabular}{l|cc|cc}
  \hline
  \multirow{2}{*}{Method} & \multicolumn{2}{c|}{MS-COCO} & \multicolumn{2}{c}{Flickr30K} \\ 
           & R@1  & R@5  & R@1  & R@5  \\ \hline
InternVL-C & 54.1 & 77.1 & 82.1 & 96.0 \\
DFN-H/378  & 55.6 & 79.2 & 82.1 & 96.0 \\
\rowcolor{tl!50} \adjustbox{valign=c}{\includegraphics[width=0.02\linewidth]{tables/logo.png}} Ours & \textbf{55.6} & \textbf{80.3} & \textbf{84.9} & \textbf{96.7} \\  \hline
 \end{tabular}
}
 \label{tab:ret_t2i}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\centering
 \centering
  \caption{\textbf{Zero-shot text-to-audio retrieval. } }
\resizebox{\linewidth}{!}{
 \begin{tabular}{l|cc|cc}
  \hline
  \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Clotho} & \multicolumn{2}{c}{Audiocaps} \\ 
               & R@1  & R@10 & R@1  & R@10  \\ \hline
LanguageBind-H & 16.7 & 52.0 & 19.7 & 67.6  \\
InternVideo2\textrm{-6B}  & 17.4 & -    & \textbf{37.1} & - \\
\rowcolor{tl!50} \adjustbox{valign=c}{\includegraphics[width=0.02\linewidth]{tables/logo.png}} Ours 
               & \textbf{17.6} & \textbf{52.2} & 23.0 & \textbf{69.4}  \\  \hline
 \end{tabular}
}
 \label{tab:ret_t2a}
\end{minipage}
\end{table}
\endgroup

==> tables/stal_param.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}
\centering
\caption{\textbf{Hyper-parameters for STAL.}}
\label{table:stal_param}
\begin{tabular}{ll}
\hline
  Hyperparameters & AVA v2.2  \\ \hline
\multicolumn{1}{l}{\it{\textbf{Decoder architecture}}} \\ \hline
\# of layers & 6   \\
Hidden size  & 256 \\
MLP dimension   & 2048   \\
Box head \# layers & 3   \\
Dropout rate & 0.1 \\ \hline
\multicolumn{1}{l}{\it{\textbf{Training}}} \\ \hline
Optimizer & AdamW  \\
Optimizer momemtum & $\beta_1=0.9$, $\beta_2=0.999$ \\
Weight decay & 1e-5   \\
Learning rate   & 1e-4   \\
Batch size   & 256 \\
Warmup epochs   & 10  \\
Epochs & 50  \\
Drop path & 0.1 \\ \hline
\end{tabular}
\end{table}



% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{lll}
% \hline
%   & Config & AVA v2.2  \\ \hline
% \multirow{5}{*}{Decoder architecture} & \# of layers & 6   \\
%   & Hidden size  & 256 \\
%   & MLP dimension   & 2048   \\
%   & Box head \# layers & 3   \\
%   & Dropout rate & 0.1 \\ \hline
% \multirow{8}{*}{Training} & Optimizer & AdamW  \\
%   & Optimizer momemtum & $\beta_1=0.9$, $\beta_2=0.999$ \\
%   & Weight decay & 1e-5   \\
%   & Learning rate   & 1e-4   \\
%   & Batch size   & 256 \\
%   & Warmup epochs   & 10  \\
%   & Epochs & 50  \\
%   & Drop path & 0.1 \\ \hline
% \end{tabular}
% \end{table}
